MUST-VQA: MUltilingual Scene-text VQA

In this paper, we present a framework for Multilingual Scene Text Visual Question Answering that deals with new languages in a zero-shot fashion. Specifically, we consider the task of Scene Text Visual Question Answering (STVQA) in which the question can be asked in different languages and it is not necessarily aligned to the scene text language. Thus, we first introduce a natural step towards a more generalized version of STVQA: MUST-VQA. Accounting for this, we discuss two evaluation scenarios in the constrained setting, namely IID and zero-shot and we demonstrate that the models can perform on a par on a zero-shot setting. We further provide extensive experimentation and show the effectiveness of adapting multilingual language models into STVQA tasks.

==> tables/stvqa-only_english.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\begin{tabular}{llccc}
\hline
\rowcolor[HTML]{FFFFFF} 
Models        & OCR System    & No. of Params & Val Acc.       & Val ANLS       \\ \hline
\rowcolor[HTML]{FFFFFF} 
M4C           & Microsoft-OCR                & 200M          & 38.05          & 0.472          \\
\rowcolor[HTML]{FFFFFF} 
SA-M4C        & Microsoft-OCR             & 200M          & 42.23          & 0.512          \\
\rowcolor[HTML]{FFFFFF} 
SMA           & Microsoft-OCR            & -             & -              & -              \\
\rowcolor[HTML]{FFFFFF} 
LaAP-Net      & Microsoft-OCR              & -             & 39.74          & 0.497          \\
\rowcolor[HTML]{FFFFFF} 
LOGOS         & Microsoft-OCR            & -             & 48.63          & 0.581          \\
\rowcolor[HTML]{FFFFFF} 
TAP           & Microsoft-OCR                & 200M          & 50.83          & 0.598          \\
\rowcolor[HTML]{FFFFFF} 
LaTr-base \ding{72} & Amazon-OCR               & 311M          & \textbf{58.41} & \textbf{0.675} \\
\rowcolor[HTML]{EFEFEF} 
mLaTr\_base   & Microsoft-OCR               & 586M          & 48.71          & 0.5831         \\
\rowcolor[HTML]{EFEFEF} 
mLaTr\_base   & Microsoft-OCR                & 586M          & 48.02          & 0.6145        
\end{tabular}
\label{tab:only-english-stvqa}
\caption{\textbf{Results on the ST-VQA dataset trained on only English}.}
\end{table}

==> tables/stvqa_translate_robustness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering

% \begin{tabular}{l |
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c |
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c }

%                                         & CA    & ES    & ZH    & IT    & EL    \\ \hline
% \cellcolor[HTML]{FFFFFF}OPUS            & 46.84 & 47.72 & 45.74 & 46.31 & 46.84 \\
% \cellcolor[HTML]{FFFFFF}M2M\_100        & 47.22 & 47.68 & 45.97 & 46.16 & 45.09 \\
% \cellcolor[HTML]{FFFFFF}mBART           & -     & 46.96 & 45.89 & 45.93 & -    
% \end{tabular}

\begin{tabular}{
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |l}
                                 & CA                            & ES                            & ZH                            & IT                            & EL                            & \textbf{Avg}   \\ \hline
OPUS                             & 46.84                         & 47.72                         & 45.74                         & 46.31                         & 46.84                         & \textbf{47.96} \\
\cellcolor[HTML]{EFEFEF}M2M\_100 & \cellcolor[HTML]{EFEFEF}47.22 & \cellcolor[HTML]{EFEFEF}47.68 & \cellcolor[HTML]{EFEFEF}45.97 & \cellcolor[HTML]{EFEFEF}46.16 & \cellcolor[HTML]{EFEFEF}45.09 & \textbf{47.96} \\
mBART                            & -                             & 46.96                         & 45.89                         & 45.93                         & -                             & \textbf{47.96}
\end{tabular}

\caption{\textbf{Results on STVQA dataset}. Results refer to \textit{mLaTr-base} with visual features and Microsoft-OCR. Its Avg. Acc. on Original ML-STVQA questions is \textbf{47,96\%}. STVQA questions have been translated into the 5 languages using OPUS, M2M100 (1.2B), and mBART.}
\label{tab:STVQA-translate-robust}
\end{table}

==> tables/textvqa-only_english.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\begin{tabular}{llcc}
\hline
\rowcolor[HTML]{FFFFFF} 
Models        & OCR System    & No. of Params & Val Acc.       \\ \hline
\rowcolor[HTML]{FFFFFF} 
M4C           & Microsoft-OCR & 200M          & 45.22          \\
\rowcolor[HTML]{FFFFFF} 
SA-M4C        & Microsoft-OCR & 200M          & 45.4           \\
\rowcolor[HTML]{FFFFFF} 
SMA           & Microsoft-OCR & -             & -              \\
\rowcolor[HTML]{FFFFFF} 
LaAP-Net      & Microsoft-OCR & -             & 40.68          \\
\rowcolor[HTML]{FFFFFF} 
LOGOS         & Microsoft-OCR & -             & 51.53          \\
\rowcolor[HTML]{FFFFFF} 
TAP           & Microsoft-OCR & 200M          & 49.91          \\
\rowcolor[HTML]{FFFFFF} 
LaTr-base \ding{72} & Amazon-OCR    & 311M          & \textbf{61.05} \\
\rowcolor[HTML]{EFEFEF} 
mLaTr\_base   & Microsoft-OCR & 586M          & 46.63          \\
\rowcolor[HTML]{EFEFEF} 
mLaTr\_base   & Microsoft-OCR & 586M          & 48.02         
\end{tabular}
\label{tab:only-english-textvqa}
\caption{\textbf{Results on the Text-VQA dataset trained on only English}.}
\end{table}

==> tables/textvqa_translate_robustness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[]
% \centering
% \begin{tabular}{l
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c |
% >{\columncolor[HTML]{FFFFFF}}c 
% >{\columncolor[HTML]{FFFFFF}}c }
%                                  & CA    & ES    & ZH    & IT    & EL    \\ \hline
% \cellcolor[HTML]{FFFFFF}OPUS     & 42,25 & 45,73 & 43,82 & 44,53 & 43,39 \\
% \cellcolor[HTML]{FFFFFF}M2M\_100 & 45,73 & 45,69 & 44,39 & 44,91 & 43,29 \\
% \cellcolor[HTML]{FFFFFF}mBART    & -     & 45,76 & 43,53 & 44,81 & -   
% \end{tabular}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{lccc|cc|c}
         & \cellcolor[HTML]{FFFFFF}CA & \cellcolor[HTML]{FFFFFF}ES & \cellcolor[HTML]{FFFFFF}ZH & \cellcolor[HTML]{FFFFFF}IT & \cellcolor[HTML]{FFFFFF}EL & \cellcolor[HTML]{FFFFFF}\textbf{Avg} \\ \hline
\rowcolor[HTML]{FFFFFF} 
OPUS     & 42.25                      & 45.73                      & 43.82                      & 44.53                      & 43.39                      & \cellcolor[HTML]{FFFFFF}\textbf{46.06}     \\
\rowcolor[HTML]{EFEFEF} 
M2M\_100 & 45.73                      & 45.69                      & 44.39                      & 44.91                      & 43.29                      & \textbf{46.06}                             \\
\rowcolor[HTML]{FFFFFF} 
mBART    & /                          & 45.76                      & 43.53                      & 44.81                      & /                          & \cellcolor[HTML]{FFFFFF}\textbf{46.06}    
\end{tabular}
\caption{\textbf{Results on TextVQA dataset}. Results refer to \textit{mLaTr-base} without visual features and Microsoft-OCR. Its Avg. Accuracy on Original ML-TextVQA questions is \textbf{46.06\%}. TextVQA questions have been translated into the 5 languages using OPUS, M2M100 (1.2B), and mBART.}
\label{tab:TextVQA-translate-robust}
\end{table}
